Learned Nonlinear Predictor for Critically Sampled 3D Point Cloud Attribute Compression

We study 3D point cloud attribute compression via a volumetric approach: assuming point cloud geometry is known at both encoder and decoder, parameters $\theta$ of a continuous attribute function $f: \mathbb{R}^3 \mapsto \mathbb{R}$ are quantized to $\hat{\theta}$ and encoded, so that discrete samples $f_{\hat{\theta}}(\mathbf{x}_i)$ can be recovered at known 3D points $\mathbf{x}_i \in \mathbb{R}^3$ at the decoder. Specifically, we consider a nested sequences of function subspaces $\mathcal{F}^{(p)}_{l_0} \subseteq \cdots \subseteq \mathcal{F}^{(p)}_L$, where $\mathcal{F}_l^{(p)}$ is a family of functions spanned by B-spline basis functions of order $p$, $f_l^*$ is the projection of $f$ on $\mathcal{F}_l^{(p)}$ represented as low-pass coefficients $F_l^*$, and $g_l^*$ is the residual function in an orthogonal subspace $\mathcal{G}_l^{(p)}$ (where $\mathcal{G}_l^{(p)} \oplus \mathcal{F}_l^{(p)} = \mathcal{F}_{l+1}^{(p)}$) represented as high-pass coefficients $G_l^*$. In this paper, to improve coding performance over \cite{do2023volumetric}, we study predicting $f_{l+1}^*$ at level $l+1$ given $f_l^*$ at level $l$ and encoding of $G_l^*$ for the $p=1$ case (RAHT($1$)). For the prediction, we formalize RAHT(1) linear prediction in MPEG-PCC in a theoretical framework, and propose a new nonlinear predictor using a polynomial of bilateral filter. We derive equations to efficiently compute the critically sampled high-pass coefficients $G_l^*$ amenable to encoding. We optimize parameters in our resulting feed-forward network on a large training set of point clouds by minimizing a rate-distortion Lagrangian. Experimental results show that our improved framework outperforms the MPEG G-PCC predictor by $11\%$--$12\%$ in bit rate.

==> two_pages_for_GSAL.tex <==
\section{Introduction}
\label{sec:intro}

We study lossy compression of 3D point cloud attributes from a volumetric function approach.
Specifically, assuming point cloud \textit{geometry} is first encoded, we encode point cloud \textit{attributes}, given that encoded geometry is known both at encoder and decoder \cite{GPCC:20}. 
Mathematically, given known 3D locations $\x_i \in \mathbb{R}^3$ both at encoder and decoder, we encode quantized parameters $\hat{\theta}$ for a target volumentric attribute function $f: \mathbb{R}^3 \mapsto \mathbb{R}$ from coarse to fine resolutions for scalability, so that it can be evaluated as $f_{\hat{\theta}}(\x_i)$ at known $\x_i$ at the decoder for signal reconstruction. 
\cite{QueirozC:16} proposed such a framework called \textit{Region Adaptive Hierarchical Transform} (RAHT(1)), and now forms the core in MPEG G-PCC \cite{ChouKK:20}. 
Recently, \cite{do2023volumetric, do2024volumetric} extended this framework to B-spline basis functions of higher order and demonstrated significant coding gain. 
Moreover, the feedforward network obtained by unrolling a finite-term Taylor's series of a matrix inverse to compute coefficients of orthonormalized basis vectors for RAHT($p>1$) is amenable to end-to-end data-driven parameter tuning. 

In addition, we further improve performance by designing a predictor for finer-grained coefficients $F_{l+1}^*$ given coarser-grained coefficients $F_l^*$. 
In particular, stemming from the seminal \textit{bilateral filter} (BF) \cite{tomasi98} in image denoising, we propose a \textit{polynomial bilateral filter} (PBF) that is a signal-dependent \textit{pseudo-linear} filter for finer-grained coefficient prediction. 
PBF has been shown in \cite{antonio2013polybf} to possess a graph spectral low-pass filter interpretation that is common in the \textit{graph signal processing} (GSP) liteature \cite{ortega18ieee,cheung18}.
% Leveraging the feedforward charcteristic of the developed network \cite{do2023volumetric, do2024volumetric}, we train the coefficients of PBF and other network parameters in a data-driven manner for optimal prediction. 
Experimental results show that PBF's predictive performance outperforms a linear predictor inspired by MPEG standardization for a wide range of point cloud datasets.

% The outline of the paper is as follows.
% We first overview the coding framework in Section\;\ref{sec:framework}.
% We describe our proposed predictor and prediction residual coding in Section\;\ref{sec:implement}.
% Finally, we present experimental results and conclusion in Section\;\ref{sec:results} and \ref{sec:conclude}, respectively.


\begin{figure}[t]
    \centering
    % trim=left bottom right top, clip
    % \begin{subfigure}{0.2\textwidth}
    %     \centering
    %     \includegraphics[width=\linewidth,trim=7.0in 5.0in 7.0in 2.5in,clip]{ICASSP24/Figures/Original00.png}
    %     \caption{}
    % \end{subfigure}
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth,trim=9.5in 8in 8.3in 3.8in,clip]{Figures/Raht1_actual01.png}
        \caption{}
    \end{subfigure}
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth,trim=9.5in 8in 8.3in 3.8in,clip]{Figures/Raht1_linear02_marked.png}
        \caption{}
    \end{subfigure}
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth,trim=9.5in 8in 8.3in 3.8in,clip]{Figures/Raht2_gbf03_marked.png}
        \caption{}
    \end{subfigure}
    \vspace{-0.05in}
    \caption{Point cloud encoded at $0.325$bpp: (a) Naive RAHT($p=1$); (b) RAHT($p=1$) + linear; (c) Our model RAHT($p=2$) + PBF.}
    \label{fig:reconstructed_PCs}
\end{figure}


\begin{figure*}[t]
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth,trim=0.05in 0.0in 0.05in 0.0in,clip]{Figures/Result_ICAPPS24_-_Longdress_-_smalllines.png}
        \caption{}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth,trim=0.05in 0.0in 0.05in 0.0in,clip]{Figures/Result_ICAPPS24_-_Redandblack_-_smalllines.png}
        \caption{}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth,trim=0.05in 0.0in 0.05in 0.0in,clip]{Figures/Result_ICAPPS24_-_Loot_-_smalllines.png}
        \caption{}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth,trim=0.05in 0.0in 0.05in 0.0in,clip]{Figures/Result_ICAPPS24_-_Soldier_-_smalllines.png}
        \caption{}
    \end{subfigure}
    \vspace{-0.05in}
    \caption{Rate-Distortion  curves: (a) \textit{Longdress}, (b) \textit{Redandblack}, (c) \textit{Loot}, (d) \textit{Soldier}}
    \label{fig:code_gain_performance}
\vspace*{-2ex}
\end{figure*}

\vspace*{-0.5ex}
\section{Coding Framework}
Denote by $f:\mathbb{R}^3\mapsto\mathbb{R}$ a volumetric function defining an attribute field over $\mathbb{R}^3$.
Then, a point cloud can be seen as samples of $f$, with attributes $y_i=f(\mathbf{x}_i)$, where $\x_i \in \mathbb{R}^3$ is sample $i$'s 3D position. 
In \cite{do2023volumetric}, RAHT($p$) codes the attributes given the positions by projecting $f$ onto a nested sequence of function spaces $\mathcal{F}_{l_0}^{(p)}\subseteq\cdots\subseteq\mathcal{F}_L^{(p)}$. 
Each function space $\mathcal{F}_l^{(p)}$ is a parametric family of functions spanned by a set of basis functions $\{\phi_{l,\mathbf{n}}^{(p)}:\mathbf{n}\in\mathcal{N}_l\}$, namely the volumetric B-spline basis functions $\phi_{l,\mathbf{n}}^{(p)}(\mathbf{x})=\phi_{0,\mathbf{0}}^{(p)}(2^l\mathbf{x}-\mathbf{n})$ of order $p$ and scale $l$ for offsets $\mathbf{n}\in\mathcal{N}_l\subset\mathbb{Z}^3$.
The results are the projections $f_l^*$ of $f$ on $\mathcal{F}_l$ and the prediction residual functions between consecutive projections, defined as $g_l^{\ddagger}=f_{l+1}^*-\text{pred}(f_l^*)$, where the gap between levels of details ($l$ and $l+1$) is reduced by incorporating an up-sampling prediction operation $\text{pred}(.)$. 
Thus, we can write
\vspace{-1.3ex}
\begin{eqnarray}
f_L^* & = & \text{pred}(f_{l_0}^*) + g_{l_0+1}^{\ddagger} + \cdots + g_l^{\ddagger} + \cdots + g_{L-1}^{\ddagger} .
\vspace{-2.4ex}
\label{eqn:fg0_gL}
\end{eqnarray}
 
We assume that resolution $L$ is high enough such that $f_L^*(\mathbf{x}_i)=f(\mathbf{x}_i)$.
We code $f$ by coding $f_{l_0}^*$, $g_{l_0+1}^{\ddagger},\ldots,g_{L-1}^{\ddagger}$.  
These functions are represented as coefficients in a basis, which are quantized and entropy coded.  
It is showed in \cite{do2023volumetric, do2024volumetric}  how to compute these coefficients efficiently. 

% Denote by $\mathcal{G}_l$ the orthogonal complement subspace to $\mathcal{F}_l$ in $\mathcal{F}_{l+1}$. 
% Then, we can write
% \vspace{-1.3ex}
% \begin{eqnarray}
% \cF_L & = &\cF_{l_0} \oplus \cG_{l_0+1} \oplus \cdots \oplus \cG_l \oplus \cdots \cG_{L-1}   \;\;\; \mbox{and}
% \label{eq:sum_of_subspaces} \\
% f_L^* & = & f_{l_0}^* + g_{l_0+1}^* + \cdots + g_l^* + \cdots + g_{L-1}^* .
% \vspace{-2.4ex}
% \label{eqn:fg0_gL}
% \end{eqnarray}
% We assume that the resolution $L$ is high enough such that $f_L^*(\mathbf{x}_i)=f(\mathbf{x}_i)$.
% We then code $f$ by coding $f_{l_0}^*$, $g_{l_0+1}^*,\ldots,g_{L-1}^*$.  
% These functions are represented as coefficients in a basis, which are quantized and entropy coded.  
% \cite{do2023volumetric} showed how to compute these coefficients efficiently. 


\subsubsection{Low-pass Coefficients}

Denote by $\bPhi_l=[\phi_{l,\mathbf{n}}]$ the row-vector of basis functions at level $l$, and by $\bPhi_l^\top=[\langle\phi_{l,\mathbf{n}},\cdot\rangle]$ the column-vector of functionals that are inner products with the basis functions at level $l$. 
Then, $\bPhi_l^\top f=[\langle\phi_{l,\mathbf{n}},f\rangle]$ is the column-vector of inner products of the basis functions with $f$, and $\bPhi_l^\top\bPhi_l$ is the matrix of inner products of the basis functions with themselves, namely the \textit{Gram matrix}. 
Here, the inner product is given by $\langle g,f\rangle=\sum_ig(\mathbf{x}_i)f(\mathbf{x}_i)$.

Further, denote by $f_l^*$ the projection of the function $f$ onto the subspace $\mathcal{F}_l$, and by $F_l^*$ its coefficients in the basis $[\phi_{l,\mathbf{n}}]$, i.e., $f_l^*=\bPhi_{l,\mathbf{n}}F_l^*$.  The coefficients $F_l^*$, which we call {\em low-pass coefficients}, can be determined via a solution of the normal equations, \ie, 
\vspace{-1ex}
\begin{equation} \label{eq:normal_equation_F}
F_{l}^* = (\bPhi_{l}^{\top} \bPhi_{l})^{-1} \bPhi_{l}^{\top} f .
\vspace{-1ex}
\end{equation}

\subsubsection{Residual coefficients}
\label{sec:residual_coding}
In the latest work \cite{do2024volumetric}, we represent the residual prediction function $g_l^{\ddagger}$ in the basis $\bPhi_{l+1}$. 
In this basis, the coefficients for $g_l^{\ddagger}=f_{l+1}^*-\text{pred}(f_l^*)=\bPhi_{l+1}F_{l+1}^*-\bPhi_{l+1} \P_l^\top F_l^*$ are given by (\ref{eq:normal_equation_F}), and $\P_l^\top$ is an up-sampling prediction operator.  
Its input is the low-pass coefficients $F_l^*$ from lower level of detail. Hence, the {\em residual coefficients} are defined as
\vspace{-1ex}
\begin{equation}
    (\bPhi_{l+1}^\top\bPhi_{l+1})^{-1}\bPhi_{l+1}^\top g_l^{\ddagger} = F_{l+1}^*-\P_l^\top F_l^* \stackrel{\Delta}{=} \delta F_{l+1}^{\ddagger} .
    \label{eqn:delta_F}
\vspace{-0.5ex}
\end{equation}

As done in \cite{do2024volumetric}, instead of quantizing the coefficients $F_l^*$ or $\delta F_{l+1}^{\ddagger}$ directly, we \textit{orthonormalize} them first as
\vspace{-1ex}
\begin{align}
    \bar{F}_{l}^* &
    % = (\bPhi_{l}^{\top} \bPhi_{l})^{-\frac{1}{2}} \bPhi_{l}^{\top} f
    = (\bPhi_{l}^{\top} \bPhi_{l})^{\frac{1}{2}} F_l^* \label{eqn:orthor_normal_equation_F} \;\;\;\mbox{and} \\
    \delta \overline{F}_{l+1}^{\ddagger}  &
    % = (\bPhi_{l+1}^{\top} \bPhi_{l+1})^{-\frac{1}{2}} \bPhi_{l+1}^{\top} g_{l}^*
    = (\bPhi_{l+1}^{\top} \bPhi_{l+1})^{\frac{1}{2}} \delta F_{l+1}^{\ddagger} .
\label{eq:orthor_normal_equation_G}
\end{align}
To compute \eqref{eqn:orthor_normal_equation_F} and \eqref{eq:orthor_normal_equation_G}, we implement the operator $\X^{\frac{1}{2}} = \X^{-\frac{1}{2}} \X$ as a $P$-layer feedforward network with coefficients initially derived from the $P$th order Taylor expansion of $x^{-\frac{1}{2}}$.


% \subsubsection{Polynomial Bilateral Filter Prediction}
% Next, we introduce another enhancement operation from \cite{antonio2013polybf}, the \textbf{polynomial bilateral filter} (PBF). The PBF is a polynomial version of the {\em bilateral filter} (BF).  As is well known, the our BF is defined as the weights in the the 27-neighborhood $\mathcal{M}(i)$ of node $i$ 
% \begin{equation}
% w_{\mathbf{k}_{ij}} = \exp \left( -\frac{\| \mathbf{n}_i-\mathbf{n}_j \|^2}{2\sigma_x^2} \right) \, \exp \left( -\frac{\| \mathbf{x}[i]-\mathbf{x}[j] \|^2}{2\sigma_y^2} \right) ,
% \end{equation}
% where $\sigma_x$ and $\sigma_y$ are the filter parameters, which may be trained.
% Then, the bilateral filter can then be generalized into a graph filter with spectral response function belonging to the class of polynomial functions with maximum degree $K$,
% \begin{align}
%     \textit{h}(\boldsymbol{\mathcal{L}}_r) &= r_0 \prod_{k=0}^{K} (\mathbf{I} - r_k \boldsymbol{\mathcal{L}}_r) , \\
%     \mbox{\it PBF}(\mathbf{x}) &= \textit{h}(\boldsymbol{\mathcal{L}}_r) \mathbf{x} .
%     \label{eq:polynomials_BF}
% \end{align}
% The polynomials coefficients $\{ r_k\}_{k=0}^K$ may be trained.


\vspace*{-0.5ex}
\section{Experiments}
\subsubsection{Setup}
Our training dataset comprises voxelized point clouds derived from 3D models (meshes) publicly available in sketchfab\footnote{https://sketchfab.com/blogs/community/sketchfab-launches-public-domain-dedication-for-3d-cultural-heritage/}. 
% We picked 10 meshes that resemble the human form and densely sampled points on the faces of the meshes, calculated the points' colors from the provided UV texture map, and voxelized the points by quantizing the point positions into voxels and averaging the point colors in each voxel.
Our evaluation dataset comprises the MPEG point clouds \textit{Longdress}, \textit{Redandblack}, \textit{Loot}, and \textit{Soldier} \cite{dEonHMC:2017}.
All point clouds have 10-bit resolution, so their octrees have depth of $L=10$ and $N_L \sim  1e^6$.
Lastly, we use the adaptive Run-Length Golomb-Rice (RLGR) entropy coder to calculate a realizable bit rate. 

\subsubsection{Results}

For our models, we first initialize the parameters such that they correspond to volumetric B-splines of order $p=2$, namely RAHT($p=2$). For the up-sampling prediction, we test the \textit{PBF} predictor along with a simple locally linear weighted average interpolation scheme. Here, before any training process, we are able to initialize the model parameters to attain reasonable performance, then the training will only improve the performance further.

Our coding improvements over the baseline model are largely attributable to the higher B-spline order, RAHT($p=2$), coupled with prediction. 
This is expected, because the representations at scale $l$ are the \textit{piecewise trilinear} functions of RAHT($p=2$), which contain more details than the \textit{piecewise constant} functions of RAHT($p=1$).  The former can be used for better prediction of the next scale $l+1$. Fig.\,\ref{fig:reconstructed_PCs} shows that blocking artifacts are much less visible with our model, especially at boundaries between objects, where there are continuous transitions of colors.
\vspace*{-0.05in}

\section{Conclusion}
\label{sec:conclude}
We extend previous works, including MPEG G-PCC, that use a volumetric approach for 3D point cloud attribute coding, by proposing a polynomial bilateral filter for predicting the upsampled signals, whose coefficients are trainable. 
